Imitation and Supervised Learning of Compliance for Robotic Assembly

We present the design of a learning-based compliance controller for assembly operations for industrial robots. We propose a solution within the general setting of learning from demonstration (LfD), where a nominal trajectory is provided through demonstration by an expert teacher. This can be used to learn a suitable representation of the skill that can be generalized to novel positions of one of the parts involved in the assembly, for example the hole in a peg-in-hole (PiH) insertion task. Under the expectation that this novel position might not be entirely accurately estimated by a vision or other sensing system, the robot will need to further modify the generated trajectory in response to force readings measured by means of a force-torque (F/T) sensor mounted at the wrist of the robot or another suitable location. Under the assumption of constant velocity of traversing the reference trajectory during assembly, we propose a novel accommodation force controller that allows the robot to safely explore different contact configurations. The data collected using this controller is used to train a Gaussian process model to predict the misalignment in the position of the peg with respect to the target hole. We show that the proposed learning-based approach can correct various contact configurations caused by misalignment between the assembled parts in a PiH task, achieving high success rate during insertion. We show results using an industrial manipulator arm, and demonstrate that the proposed method can perform adaptive insertion using force feedback from the trained machine learning models.

==> introduction.tex <==
\section{Introduction}
\label{sec:Introduction}

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{Figures/exp_assista_v1.JPG} % 
    \caption{Experimental setup with a 6 DoF manipulator in a possible contact configuration with the hole environment.}
    \label{fig:exp_setup}
\end{figure}
Mating parts under tight tolerances is one of the most important operation in robotic assembly. In industrial uses, strict repeatability of position and/or the orientation of the parts are usually assumed, so that open-loop programs can be executed correctly. Under such assumption, a fixed sequence of operations to be performed by the robot devices can be taught to it by a human operator by means of a teaching pendant. The teaching pendant stores coordinates of via points in the robot’s memory, and the via points can be traversed at run time without any modification. The less-than-perfect repeatability and trajectory tracking of robot motion can usually be handled by a compliant position controller, for example one implementing stiffness control (\cite{Lynch2017ModernRobotics}). In many cases, minimal or no further programming of the robot is needed.

However, complications arise when the positions of the parts involved in assembly vary between repetitions of the assembly operation. This can happen in a case where the parts are deposited onto a surface by a feeder, and each time end up in a different position; also, in a case where the parts arrive on a moving conveyor belt. In such cases, industrial vision cameras can be used to determine the parts’ position. However, the determined position of the parts by the industrial vision cameras is usually fairly inaccurate, often by several millimeters. This is significantly more than the required tolerances during assembly, often measured in micrometers. For this reason, standard stiffness controllers usually fail to perform the operation successfully. Besides, even if the robotic device knows the exact position of the parts, its path (via points) still needs to be modified in order to accommodate the variation in the position of the parts. In practice, such a modification is performed by means of a dedicated computer program that takes as input the changed position of the parts and outputs a new path for the robot. However, developing such a dedicated computer program is typically very difficult and laborious, and is currently one of the main contributors to the high cost of deploying and re-tooling robotic devices for new assembly operations.


Therefore, there is a strong industrial need for methods for creating robot controllers that can accommodate varying positions of assembly parts with minimal or no programming. That is, the robot controller should be able to generalize over the positions of the parts. Arguably, generalization is one of the hallmarks of intelligence, be it human or artificial, and endowing robots with the ability to generalize over the starting conditions of assembly tasks would amount to a qualitatively different type of intelligent assembly functionality. Such a functionality would match the ability of human workers to learn a new assembly skill and apply it to many new situations.  

In fact, the way humans learn to perform an assembly task and generalize over its starting conditions also suggests the principle of operation of the method described in this paper. Although a lot of basic manipulation skills are acquired by humans by means of self-exploration, typically, in a factory setting, when a human worker learns a new operation in a factory, it is usually through a demonstration given by a senior worker. In general, only a minimal number of demonstrations (even as few as only one) are sufficient in order to learn the skill. When observing a demonstration, a human worker identifies the correct parts to be mated (usually by their appearance), the general approach of the mating motion, and perhaps a suitable trajectory for bringing the parts together. Initial attempts to perform the operation might not be immediately successful --- the two parts might jam or not even connect properly. In such a case, a series of exploratory motions guided by visual and tactile sensing are attempted by the worker. Finally, human workers learn to perform the operation flawlessly and quickly, and can perform it even without looking at the parts --- ''with their eyes closed'', as the expression is. 

Certainly, this learning process relies heavily on skills that have been learned much earlier in human development, such as the ability to recognize objects and estimate their poses visually, as well as general-purpose manipulation skills and strategies involved in inserting one object into another. The method proposed in this paper is very similar in its general approach. It relies on learning from demonstration to acquire a motion that largely brings the two parts together, ending in an approach direction that is more or less aligned with the correct one. The method also uses standard industrial techniques for recognizing the parts and estimating their poses. Finally, the algorithm learns how to correct the initial trajectory based on tactile feedback by means of self-exploration, in the form of an adaptive compliance controller. 

A commonly used prototypical robot assembly operation is the insertion of a peg into a hole, and we will use this task as an example when describing and evaluating the algorithm. We are considering the version of the problem where the position of the peg and/or the hole can vary. What we desire is an algorithm that can allow a robot equipped with a camera and a force/torque sensor mounted on its wrist to learn this operation, with minimal or no programming, even when the estimates of the positions of the parts are not very precise. We assume that a human instructor can provide at least one demonstration of a successful operation, using the robot itself. 

\begin{figure*}
    \centering
    \includegraphics[width=0.85\textwidth]{Figures/Adaptive_PiH_cover.pdf} % 
    \caption{The proposed method for design of a force controller-based learning method for part assembly. The proposed method uses an accommodation controller for exploration during the sustained contact during assembly.}
    \label{fig:proposed_method}
\end{figure*}

The peg-in-hole (PiH) insertion operation has been studied extensively in the robotics literature. Section \ref{sec:RelatedWork} discusses some of this research that is relevant to the version of the problem that we are considering. Section \ref{sec:Algorithm} describes how the components of our algorithm operate and interact with each other. Section \ref{sec:experiments} describes experiments that verify the operation of the algorithm, and Section ... concludes and outlines directions for future work.

==> method.tex <==
\section{Proposed Problem Statement }
\label{sec:proposed_problem_statement}
In this section, we present the problem that we are interested in solving. We also present an analytical model which can be used to resolve the misalignment from the F/T data. We also introduce the nomenclature that we are going to use in the rest of the paper. A schematic showing a possible contact configuration during insertion with the contact forces and reference frames is shown in Figure~\ref{fig:pih_analytical}. 


From the analysis of the state of the art in the previous section, it is apparent that none of the current robot learning methods can solve the problem of learning a compliant control policy for contact-rich assembly tasks with variable start and goal states, under the conditions of significant uncertainty in the estimation of the position of the parts being assembled, and without detailed knowledge of the geometry of the parts being manipulated. For the version of the problem we are considering (lateral misalignment of several millimeters, and possibly angular misalignment of several degrees), all three situations shown in Fig. \ref{fig:configs} can be encountered. These needs suggest a solution that uses two different machine learning methods, as described below. One of these methods is to learn a nominal trajectory in the form of a DMP, and adjust it appropriately for new start and goal states. The second method is based on a form of active supervised learning that collects training examples relating various displacements of the peg from its correct position for insertion and the FT sensations observed as a result, by means of active experimentation with the peg and hole. The collected data set is used to train a predictive model, for example a neural network, that provides adaptive active compliance by correcting the nominal trajectory produced by the DMP in response to sensed forces. 

\begin{figure}
    \centering
    \includegraphics[width=0.25\textwidth]{Figures/PiH_analytical.png} % 
    \caption{A schematic showing the $1$-dimensional case for the PiH problem with the friction cone and contact forces.}
    \label{fig:pih_analytical}
\end{figure}

Learning starts by collecting one or more demonstrations of the operation by a human. This can be done either by means of teleoperating the robot, or by direct kinesthetic teaching. The result of the human demonstration(s) is one or more trajectories in Cartesian space of the end tool of the robot of the form $y(t)$, $t \in [0,T]$. The robot starts in position $y_0=y(0)$, holding the movable part (the peg) in its gripper. The goal pose of the end tool is implicitly determined by the placement of the immobile part, in this case the hole, which is affixed to a work surface. At the end of a successful execution of the assembly operation, the pose of the end-tool is considered to have assumed the goal pose $g=y(T)$. From this definition, achieving the goal pose of the end tool is equivalent to a successful execution of the assembly operation, for a given location of the immobile object (the hole). For a different future execution of this operation, either one or both of the parts (the peg and the hole)  can be located in new and different positions. 

The poses of the parts can be estimated by means of one or more cameras. Pose estimation by means of computer vision is an active area of research (\cite{Hodan2018APose}), and various methods provide different trade-offs between cost, speed, and accuracy. High-end motion capture systems can estimate 6 degree-of-freedom (DoF) poses with accuracy on the order of $0.1mm$, but require reflective tags to be attached to the objects, and are typically expensive. On the other end of the spectrum are relatively inexpensive industrial vision systems that are often limited to 3 DoF (planar) pose estimation and have much lower accuracy, on the order of several millimeters. We assume that the pose estimation module is properly calibrated with respect to the start and end of the demonstration trajectory $y(t)$, that is, $y_0$ and $g$ are indeed the estimates returned by the camera.

After one or more trajectories $y(t)$ have been recorded for the exact same position of the hole, the DMP learning algorithm is used to learn a separate DMP for each of the components of $y(t)$. This DMP is of the form of two coupled ODEs, $\dot{x}=-\gamma x$   and $\ddot{y}=\alpha[\beta(g-y)-y]+f(x,g)$, where the forcing function $f(x,g)=\frac{\sum_{i=1}^n \psi_i \omega_i}{\sum_{i=1}^n \omega_i} x(g-y_0)$ is parameterized by means of the $n$ parameters $\omega_i$ obtained through least-squares regression from the training trajectory $y(t)$. The resulting set of DMPs can generate a new desired trajectory $y_d(t)$, given a new goal position $g_d$, by integrating the DMP’s ODEs forward in time. This kind of generalization over the goal state is an essential function of DMPs. If the new desired goal state $g_d$ was indeed the correct one, then following the new desired trajectory $y_d(t)$ would presumably reach the new goal state. However, the estimate of the desired new goal state $g_d$ is usually incorrect, because this estimate depends on the new position of the hole, as described below. Any error in the estimate of the position of the hole translates into an error in $g_d$. For this reason, the control law executed by the robot needs to provide compliance. Based on the discussion of the state of the art in the previous session, our proposal is to have a control law of the form $\dot{y}=\dot{y}_d(t)+H(\tau)$, where $\tau$ is the vector of sensed forces and torque by the FT sensor, and $H$ is a non-linear mapping that produces corrections to the velocity of the robot.  Here, $H$ is a general non-linear mapping, which makes this control law a form of a generalized damper. 

The purpose of the next stage of the algorithm is to learn the mapping $H$ through self-experimentation. To this end, while the hole is still in its original position, variations $d(t)$ are introduced to one of the original trajectories $y(t)$ demonstrated by a human operator that successfully completed the operation. If contact forces $\tau_i=\tau(t_i)$ at time $t_i$ are registered, when the velocity was varied by $d_i=d(t_i)$, the pair $(\tau_i, d_i)$ is added to a database of training examples. When a sufficient number $N$ of training examples are collected, a supervised machine learning algorithm can be used to learn the mapping between forces and the displacements that caused them. However, based on the understanding that the mapping from displacements to forces is typically many-to-one (multiple displacements would sometimes result in the same force), following the analysis in \cite{Newman2001InterpretationAssembly}, the inverse mapping would be one-to-many, that is, not a function that can be learned by means of machine learning. However, it can be realized that the exact magnitude of the displacement does not need to be recovered for successful corrective action, and furthermore, multiple displacements can generate the same forces only if the sign of these displacements is the same, as long as the magnitude of the displacement does not exceed the radius $R$ of the object being inserted. Based on this realization, a supervised machine learning algorithm can be used to learn the mapping  $sign(d_i)=H_0 (\tau_i)$, for all examples $i=1,N$ such that $|d_i |\leq R$. When the radius $R$ of the inserted object is known, it can be provided to the learning algorithm. When it is not, it can be found by searching for the largest value of $R$ that would result in a good fit on the training set with the above limitation on the magnitude of the displacement. After the mapping $H_0 (\tau)$ has been learned, the desired mapping $H(\tau)$ can be obtained by simply scaling it by a suitable velocity constant $v_0$: $H(\tau)=v_0 H_0 (\tau)$.  

\begin{figure*}
    \centering
    \includegraphics[width=0.89\textwidth]{Figures/accommodation_steady_state_plots.png} % 
    \caption{This plot shows the convergence of contact wrench obtained using the proposed GAC during a contact configuration during an insertion attempt.}
    \label{fig:accommodation_controller_plot}
\end{figure*}
At this point, it is not clear what the best way to introduce variations $d(t)$ might be. A simple way to guarantee that some contact force would be experienced would be to introduce a variation $d(T)$ to the original goal state $g$, and have the DMP algorithm generate a new trajectory $y_{mod}(t)$ that would move the peg from the original starting state $y_0$ to the modified goal state $g+d(T)$, if there was no collision between the peg and the surface. In that case, the equivalent displacements would be $d(t)=y_{mod}(t)-y(t)$. For a finite $d(T)$, a collision between the peg and the surface (or inner walls of the hole) will occur, at some time $t$. Then, if contact forces $\tau(t)$ are experienced at that time, the pair $(\tau(t),d(t))$ can be added to the training database, and the process repeated again with a new modification to the goal state until enough training examples are collected.

An alternative method for introducing variations is to generate a random displacement $d(t_1)$ at an arbitrary point in time $t_1$. If the reference trajectory is a velocity profile (and not a position profile), this variation will persist in time, that is, $d(t)=d(t_1)$ for all $t>t_1$, and will also result in a collision with the surface (or large lateral contact forces, if the variation is at a time after the peg has entered the hole).

A practical consideration about the exploration method is how to do it safely. If the robot is commanded to follow the modified trajectory in a standard position control mode, the resulting collision will either damage the robot or the parts, or result in a fault due to excessive force. This means that the robot needs to be controlled in a compliant control mode.

A similar consideration arises when the learned generalized damping control law $\dot{y}=\dot{y}_d(t)+H(\tau)$ is executed for a new desired trajectory $\dot{y}_d(t)$ generated by the DMP. If the mapping $H(\tau)$ is correct, it should be able to null out the experienced contact forces on its own. In practice, this might not always be the case, and furthermore, the control loop of the generalized damper might be too slow to react fast enough to control large contact forces. For these reasons, it might be better to command the corrected velocity $\dot{y}(t)$ to a low-level compliant controller, so that it itself can be corrected further at high control rates, if necessary. In that case, the interaction of the two compliant controllers needs to be analyzed and understood.    


==> related_work.tex <==
\section{Related Work}
\label{sec:RelatedWork}
Research on robotic assembly has a long history, and a lot of this research has used PiH insertion as a prototypical task. The main reason this task is difficult to automate is that when the peg and hole are in contact, even a small misalignment between their correct positions would cause a controller that tracks a desired trajectory defined in terms of robot positions or applied torques at the joints to result in very large contact forces that might break the robot and/or the parts. This means that open-loop execution of such trajectories is not a good solution. What is needed is a method that adjusts the motion of the parts in response to contact forces. Such techniques are also known as {\em adaptive assembly strategies} (AAS) (\cite{Nevins1977ResearchAutomation}). Some AAS can be passive, implemented by means of spring-loading the parts in their fixtures, or using specialized devices that provide compliance, such as the remote center of compliance (RCC, \cite{Nevins1977ResearchAutomation}). Other AAS are active, implemented by means of a closed-loop controller that senses forces and adjusts motion based on them. Some AAS rely on careful (and laborious) programming of the robot, wheareas others replace programming with offline planners (that still produce feedback controllers). Another class of AAS use forms of machine learning, such as imitation learning, reinforcement learning, and iterative learning for control. 

A well-known passive AAS is the Remote Center of Compliance (RCC) device, invented by Paul Watson at Draper Labs in 1976 and patented in 1979 (explained in Whitney (1982), along with why it reduces forces during mating, as well as in Nevins and Whitney (1977)). It is still in widespread use today, but has limits on its performance wrt the magnitude and type of uncertainty. It can be used well with chamfered holes, where the contact with the slope of the chamfer can bend the elastic slabs in the RCC in the appropriate direction. Passive compliance can also be implemented by the low-level controller of the robot, and most industrial robot vendors (including MELCO) do provide such stiffness controllers. However, a passively compliant device can only react to a force (or moment) by a displacement (or rotation) in the force's (or moment's) direction. That is, if the peg experiences a vertical force due to colliding with the edge of the hole, a passively compliant device cannot generate a horizontal motion towards the center of the hole. For such cases, an active interpretation of the FT signals and generation of corrective motions based on them is needed. 

The idea to use force sensing in a closed loop appeared as early as the 1970s in the US and Japan (\cite{Groome1972ForceThesis,Inoue1971ComputerManipulator}). A basic form of force sensing is to measure the applied torques at the motors, and infer from these measurements whether the robot is experienced contact with the environment. The pioneering work of Prof. Inoue (\cite{Inoue1971ComputerManipulator}) in 1971 used such measurements (and, interestingly, and early robot arm with 7 DoF manufactured by MELCO), in combination with switches mounted at the gripper of the robot. However, such torque measurements combine the torques needed to move the robot to a desired position and keep it there with the torques arising from contacts between the end tool and the environment, and separating them is not always easy or even possible. 

More commonly, contact forces are sensed by means of a dedicated force sensor that can be mounted either on the wrist of the robot, or (less often) under the platform that the hole is placed on. It returns a 6-dimensional vector consisting of 3 linear forces and 3 torques (twisting moments) along and around the three Cartesian axes. A robot controller that actively regulates what kind of forces are applied by the workpiece to the environment is known as a force controller (\cite{Lynch2017ModernRobotics}). In practice, a PiH task requires a hybrid motion-force controller, because the two parts need to move freely in some dimensions, while forces in other dimensions are being regulated. Inoue is credited with proposing and implementing the first hybrid controller \cite{Inoue1971ComputerManipulator}. 

The earliest such controllers for the PiH task were programmed manually, and were generally task-specific, with some reuse of common modules. Inoue proposed an entire language for describing manipulation operations consisting of primitive operations that can be parameterized as needed, and combined into more complex manipulation programs. Some of the primitive operations are executed in hybrid control mode, while others check for logical conditions, or move the robot freely in space \cite{Inoue1971ComputerManipulator}. A relatively complicated primitive is the one that searches for the hole by executing a search pattern while maintaining contact between the peg and the hole. Another essential primitive of the same kind is the insertion of the peg into the hole while responding to contact forces.    

A similar later example of a programming solution is Inoue's controller for a difficult insertion problem that he developed while visiting MIT's AI Lab in 1974 (\cite{Inoue1974ForceTasks}. Successful insertion of a peg in a hole with tight tolerances (0.02mm) was achieved by carefully programming the operation of the robot in response to FT readings. He proposed the use of approaching motion, until force is registered, followed by compliant motion, until the task is complete. Although impressive achievements at the time, it was clear that manual programming of force control required exceptional skill, expertise, and effort. A more general controller for insertion tasks was needed.  

Around the same time, Groome (\cite{Groome1972ForceThesis}) proposed a method for force-feedback control for contact manipulation tasks that is based on two control loops, and in many cases does not require explicit programming. The idea is to use an outer control loop that follows a position (or velocity) trajectory, and an inner control loop that follows a force profile, and corrects the trajectory followed by the outer loop based on sensed force. The general goal of the corrections is to cancel excessive undesirable forces. Groome proposed to use the experienced forces to introduce a correcting rotation around a suitable chosen ''control point'', which is usually, but not always, the point of contact. The method was successful in performing PiH insertions after the peg was brought into contact with the opening of the hole.

The idea to use an inner control loop that uses force measurements to compute corrections to an outer position or rate servo loop has been very influential, and has served as the foundation of many control methods, including the one proposed in this paper. It follows the basic principle of feedback control --- if we think of experienced excessive forces as an undesirable error, the system reacts to them so as to eliminate them, while simultaneously following a desired reference trajectory. One fundamental question related to this approach is how to compute the initial desired trajectory for the outer loop. Another one is how the corrections to this trajectory should be made as a function of sensed forces.

A practical general type of control for PiH tasks based on this principle is impedance control, where the robot is made to behave as a virtual mass, spring, and/or damper system in response to contact forces. An example of an impedance controller is a stiffness controller (\cite{Lynch2017ModernRobotics}). Given a desired trajectory of the end tool of the robot in Cartesian space $y_d(t)$, the stiffness control law takes the form $y(t)=y_d(t)+\mathcal{A}\tau$, where $\tau$ is the 6-dimensional vector of forces measured by the force/torque (FT) sensor, and $y(t)$ is the actual trajectory followed by the robot in response to contact forces. Here, $\mathcal{A}$ is the force matrix that relates the sensed forces to modifications (adaptations) to the desired trajectory. If the matrix $\mathcal{A}$ is diagonal, its diagonal entries act as (inverse) spring constants along individual dimensions. In such a case, $\mathcal{A}$ is also known as an {\em admittance} matrix. This kind of control law is relatively easy to implement on industrial robots that typically operate in position control mode, where a sequence of target points is given to a low-level controller that computes the motor torques necessary to reach them. MELCO's industrial robots provide stiffness control mode natively, if desired spring constants are provided.  

Another example of an impedance controller is the Linear Force Feedback Strategy described in (\cite{Whitney1977ForceMotions}), also commonly called accommodation servo controller, or a damping controller. For the same given desired trajectory of the end tool of the robot in Cartesian space $y_d(t)$, its equivalent velocity profile $\dot{y}_d(t)$ can be computed. Then, the control law takes the form $\dot{y}(t)=\dot{y}_d(t)+\mathcal{B}\tau$. Here, $\mathcal{B}$ is the force matrix that relates the sensed forces to modifications (adaptations) to the {\em velocity} of the desired trajectory. When diagonal, the meaning of $\mathcal{B}$'s entries is that of (inverse) damping coefficients along individual dimensions. Correspondingly, the matrix $\mathcal{B}$ is known as an {\em accommodation} matrix. By adjusting its coefficients, the robot can be made to behave as a virtual damper. This kind of damping controller is also provided natively by MELCO's industrial robots, and can be combined with a stiffness controller.

One practical difference between a stiffness controller and a damping controller is that in some common situations arising in the PiH task, a damping controller can achieve perfect correction for misalignment (that is, full elimination of contact forces), whereas a stiffness controller cannot. Such a situation occurs, for example, when the peg is advancing along the $z$ direction, which is the true and correct axial direction of the hole, but there is misalignment between the axes of the hole and peg in the transverse direction (for example, along the $x$ axis, in the amount of $\Delta x$). If the hole is chamfered, and the bottom of the peg touches the chamfer, the force $f_x$ sensed by the FT sensor along $x$, through the corresponding diagonal entry $a_x$ of the $\mathcal{B}$, would create a modification in the negative $x$ direction, thus correcting the misalignment. Eventually, the peg will slide into the hole, but because the original desired trajectory $y_d(t)$ is consistently off in the $x$ direction due to misalignment, in order to maintain a compensation of $\Delta x$ during insertion, the peg will need to be applying a constant force on the walls of the hole in the $x$ direction in the amount of $f_x =\Delta x/a_x$.

In contrast, a damping controller would introduce a correction of $b_x f_x$ to the current velocity in response to sensed force $f_x$, and this correction will persist until the end of the insertion, unless other contact forces are sensed. In practice, the low-level controller will usually be realized in discrete time, and the desired velocity profile $\dot{y}_d(t)$ will be provided as a sequence of differences (position increments) $\Delta y_d[k]=y_d[k]-y_d[k-1]=y_d(t_k)-y_d(t_{k-1})$, where $\Delta t=t_k-t_{k-1}$ is the time step of the controller. The control law in discrete time would be $\Delta y[k]=\Delta y_d[k]+B\tau$, where the matrix $B$ is derived from the matrix $\mathcal{B}$. As long as no contact has been experienced ($\tau=0$), $\Delta y[k]=\Delta y_d[k]$ and $y[k]=y_d[k]$. As soon as contact has been made with contact force $f_x$, the control law $\Delta y[k]=\Delta y_d[k]+B\tau$ will provide a correction $\Delta x=b_x f_x$ to the relative increment $\Delta y[k]$, such that $\Delta y[k]=\Delta y_d[k]+\Delta x$. This corrected increment would result in new position $y[k+1]=y_d[k+1]+\Delta y[k]=y_d[k+1]+\Delta x$ that diverges from the original desired trajectory. However, if this correction is sufficient to eliminate contact forces, that is, if when commanding the new target point $y[k+1]$ to the robot, no contact forces are experienced, then the correction will persist, and all subsequent increments $\Delta y_d[k]$ will be applied on the already corrected trajectory. In this situation, the robot would complete the insertion without any further contact forces. For this reason, damping controllers have been used in many PiH algorithms.

This type of impedance controllers (stiffness, damper, and their combinations) can be very effective when the hole is chamfered and the misalignment does not exceed the chamfer radius (or is within the tolerance of the operation). For example, for moderate tolerances, if a highly accurate pose estimation device is used to compute the pose of the hole, following a desired trajectory in impedance control mode can be sufficient for successful insertion. This implementation is quite similar to the case when the peg and/or hole have been spring-loaded, because stiffness and damping controllers implement a virtual mass-spring system. Thus, they also subsume passive adaptive control strategies. Their use is very appealing in industrial practice, because they require no manual programming, and can be tuned by means of adjusting the spring and damping coefficients only.

However, when tolerances are tight, and the amount of misalignment exceeds them, such controllers would typically fail in the insertion operation. Using the previous example, when the axial directions of the peg and hole are perfectly aligned, and there is misalignment only along the direction of $x$, if the peg's bottom surface hits the surface of the peg outside of the chamfer, there will be no force $f_x$ along $x$ sensed, but only a twisting moment $M_y$ around the $y$ axis. If a diagonal admittance (or accommodation) matrix is used, the corresponding change would be to the angle (or angular velocity) around the $y$ axis, whereas the useful corrective action would be a linear motion along the $x$ axis. 

This and other similar examples revealed the limitations of impedance controllers with diagonal admittance and/or accommodation matrices, and eventually led to the idea of using non-diagonal matrices. Indeed, in the above example, if an off-diagonal matrix element could relate a sensed moment $M_y$ to a linear displacement along the $x$ axis, then the desired corrective behavior could be achieved (\cite{Nevins1977ResearchAutomation}). The resulting controllers with full admittance and accommodation matrices are known as generalized stiffness and damper controllers, respectively. In 1982, Peshkin (\cite{Peshkin1990ProgrammedAssembly}) proposed a method for synthesizing these matrices from a set of examples about what kind of responses (linear or rotational motion of the peg) should occur for a given vector of force/torque measurements. Because this estimation is implemented in the form of minimizing a mean-square loss function over a set of examples by means of the least-squares algorithm, the method is clearly an early form of a machine learning solution to this problem; Peshkin called his method "programmed compliance", whereas "learned compliance" would have been more appropriate.

However, the limitations of linear matrices to capture the desired relationships were revealed in 1990, when Prof. Asada from MIT showed examples where the desired response to a linear combination of two FT vectors is not a linear combination of the desired responses to each of the two vectors (\cite{Asada1990TeachingCompliance,Asada1993RepresentationNets}). This means that a linear matrix is not sufficient to encode the desired relationship between the sensed FT values and the correct displacements of the peg. Instead, a non-linear mapping is necessary, and Prof. Asada demonstrated that a neural network with a single hidden layer can be constructed from the examples compiled for a planar PiH problem, so that the mapping is exact. This work established the idea that non-linear function approximators, including neural networks, might be a good way to represent the mapping from FT readings to peg motion.

This, however, still leaves the question of how the training examples should be obtained. Analyzing PiH tasks and compiling training sets is difficult, laborious, and not very practical. To overcome this difficulty, in 1994, Gullapalli et al. (\cite{Gullapalli1994AcquiringLearning}) proposed to use reinforcement learning to find the responses. He used a reward function that rewarded progress towards the goal state (peg inserted into the hole) from the current state, while penalizing contact forces. A good solution to the problem that maximizes reward is a sequence of states that progressively brings the peg closer to the fully inserted state, while avoiding contact as much as possible. It should be noted that this is {\em not} a sequential decision problem --- rather, a suitable movement is determined independently for each state, and all movements are loaded into the same neural network, for the sake of storing them and generalizing over new, unseen states that fall between the new ones. Optimization is done by means of a variant of the REINFORCE algorithm (\cite{Williams1992SimpleLearning}). 

Although Gullapalli et al.'s method led to a very impressive solution of a PiH problem problem with tight tolerances that were orders of magnitude tighter than the accuracy (repeatability) of the used robot, this method still assumes accurate knowledge of the goal state. This is not the case for the version of the problem we are considering, where the goal state is known only very approximately, and a suitable reward function cannot be provided to guide the RL algorithm.  

As pointed above, the two main questions in devising compliant controllers for PiH tasks are how to compute the initial trajectory and how to provide corrections to it based on force feedback. Clearly, they are closely related --- the more accurate the initial trajectory, the simpler the force feedback controller can be. For example, for a relatively loose tolerance (or a chamfered hole) and a relatively accurate initial trajectory that brings the tip of the peg within the hole (or chamfer, Fig. \ref{fig:configs}c), a basic stiffness and/or damping controller would be sufficient for insertion. When the entirety of the peg is not within the hole, but at least part of it is inside (Fig. \ref{fig:configs}a), a generalized stiffness/damping controller might still work. And, for a very imprecise initial trajectory, where the peg touches the surface outside of the hole (Fig. \ref{fig:configs}b), arguably, there isn't sufficient information in the force vector alone that could be used to recover the touching point and provide corrective behavior.  

\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{Figures/PiHconfigs.png} % 
    \caption{Some possible contact configurations between a peg and a hole.}
    \label{fig:configs}
\end{figure}

Research on PiH usually distinguishes clearly between the first two cases (when all or part of the bottom of the peg is in the hole at the time of initial contact), and the third case, when there is no overlap. A controller that handles the first two cases is usually referred to as an insertion controller, whereas a controller that handles the third case is called a search controller, because it usually employs some kind of a spatial search strategy to find the hole. In all three cases, though, an initial trajectory for the peg must be computed in some manner. 

In the earliest research, this trajectory was programmed manually. The simplest possible trajectory is a linear motion of the peg along its axial direction. If the peg ends up within the (chamfer of) the hole, a stiffness or damping controller can usually complete the insertion. If the peg ends up in the position shown in Fig. \ref{fig:configs}a), either a new trajectory can be chosen, or a generalized compliant controller can be used. For example, Whitney (\cite{Whitney1977ForceMotions}) described a controller that computes the azimuth of the contact point along the rim of the hole, and commands motion along this azimuth toward the center of the whole. This calculation was not done by means of an accommodation controller, but externally, effectively modifying the initial nominal trajectory in addition to the modifications of the compliance controllers.  Furthermore, the peg approached the hole with a tilt, and after contact with the side of the hole was detected (probably through a large lateral force), the tilt was removed, and the peg inserted. Similarly, Gottschlich and Kak (\cite{Gottschlich1989AMating}) used a manually designed plan consisting of a sequence of straight-line compliant motions. During insertion, the motion is towards the center of the hole, and the authors showed that this direction is the same as the projection of the vector of the measured torque onto the plane of the surface, and can be computed analytically. This essentially recovers the center of the hole from FT data, and uses it in a kind of contingency plan that transitions between steps of the plan based on force data, in a way that is robust to excessive forces due to impact. The correct vertical direction of insertion is implicitly assumed to be known, and never adjusted; if jamming or wedging occurs, the plan is backtracked. 

Clearly, both of these solutions are task- and situation-specific, and moreover, neither of them would be able to handle the case in Fig. \ref{fig:configs}b. Newman et al. (\cite{Newman2001InterpretationAssembly}) proposed a method that could potentially deal with this case by identifying where outside of the hole the peg is touching the surface, by also employing the depth of movement along the direction of insertion, as well as the entire history of sensor readings, as opposed to instantaneous values only. When the peg is tilted with respect to the surface, different points on the surface would correspond to different depths. However, the tilt degree needs to be known in order to recover the touch position. This work also provided very useful analysis of the ambiguity associated with interpreting FT and position data for the purpose of recovering the relative position of the peg and the hole when they come into contact. Furthermore, this method also used a task-specific search trajectory.   

A recent example of a method that tries to estimate the correct direction of corrective motion is due to Dong and Rodriguez (\cite{Dong2019Tactile-BasedBox-Packing}, for the related task of box packing. They used a combination of CNN and LSTM networks to interpret a sequence of sensor inputs from two GelSlim sensors by mapping the 8 pairs of image frames of the sensor after impact onto the signs of misalignment, and using interpretations in a heuristic controller that corrected the insertion approach. The method was successful in generalizing on new objects, but the experimental verification was limited to only one linear and one rotational directions of misalignment. Furthermore, the insertion tolerance was fairly large (2mm), and insertion along the chosen direction of approach was done in open loop --- this is a strategy that is not likely to work well for insertion problems with tight tolerances. Still, it is indicative of recent methods for interpreting force signals for the purposes of insertion.

A much more general solution is to automatically construct the nominal trajectory, given a geometric description of the task. In 1984, Lozano-P\'erez, Mason, and Taylor (\cite{Lozano-Perez1984AutomaticRobots}) proposed what is essentially a planning approach under uncertainty in sensing and execution. Using knowledge of the geometry of the parts, pre-images of goal states are computed, such that the goal can be achieved from them by some motion. The motion is assumed to be compliant, using the generalized damper model introduced earlier by Whitney. Sequences of states are back-chained from the goal state to compute an entire plan. The method can handle systematically uncertainty in both the position of the parts as well as the actual direction of motion of the robot. A recent example of this approach is due to Nottensteiner et al. (2020), who use particle filters to represent the remaining uncertainty of the hole's position, update it in accordance with experienced contact forces, and select the next move based on that uncertainty. A major disadvantage of this approach is that correct and precise knowledge of the geometry of the parts needs to be available, which makes its use in general assembly operations difficult.      

Another principled approach to discovering good nominal trajectories is to employ machine learning techniques, including reinforcement learning (RL) and learning from demonstration (LfD). Gullapalli et al.'s previously mentioned early method (\cite{Gullapalli1994AcquiringLearning}) was an impressive example of the use of RL to solve the PiH problem. Although the main purpose of the algorithm was to learn how to react to contact forces, it was also implicitly searching for a trajectory in configuration space that would progressively bring the peg to the (known) goal position.  

After a hiatus due to ''the second AI winter'', the recent resurgence of the popularity of neural networks and reinforcement learning in machine learning research has also led to some new applications to the problem of contact-rich manipulation. Levine et al. (\cite{levine2016}) described the application of the Guided Policy Search method for reinforcement learning to learning contact-rich manipulation skills. Similar to Gullapalli’s earlier RL method, the reward/cost function used by them needs precise knowledge of the goal position, which is not feasible in the version of the problem we are considering. Furthermore, there was no significant variation in the goal position, other than that caused by unsteadily holding of the immobile part by the second had of the robot. Moreover, this method, similar to most RL methods, suffers from significant sample complexity, that is, a large number of trial-and-error epochs needed during learning. Similarly, Inoue et al. (\cite{Inoue2017DeepTasks}, not Prof. Inoue, but another researcher from IBM Japan) proposed an RL method for solving both the search and insertion variants of the PiH problem, using an LSTM network to encode the policy and an elaborately engineered reward function that again assumed that the goal state was known precisely.

Another class of robot learning methods that are typically much more sample-efficient than RL is that of learning from demonstration (LfD) methods. Several LfD methods are based on Dynamic Movement Primitives (DMP), originally proposed by Ijspeert et al. (\cite{Ijspeert2002MovementRobots,Ijspeert2013DynamicalBehaviors}). DMPs are sets of parameterized ordinary differential equations (ODE) that can generate a trajectory that will bring a system, such as a robot, from a starting state to a goal state. The shape of this trajectory can be manipulated to match a desired trajectory, for example one given by a human demonstrator, by adjusting the parameters of the ODEs through least-squares regression. Two big advantages of DMPs are that they can easily adapt the generated trajectory to new starting as well as goal states, thus constituting essentially a closed-loop controller, and moreover, they can be learned from very few training examples, including even a single one. 

Because of this, DMP-based LfD algorithms are good candidates for solving robotic assembly problems. However, in their basic form, these algorithms cannot use force and torque measurement information to correct the generated trajectory, that is, they cannot provide the compliance needed in contact-rich applications. It is certainly possible to execute the generated trajectory by means of a compliant low-level controller, for example a standard stiffness controller, resulting in the trajectory corrections that are necessary to avoid excessive contact forces. We have achieved successful PiH insertion using this method, when the new position of the hole has been estimated accurately by means of a VICON motion tracker. However, less accurate position estimation by means of a Cognex camera has not been successful. 

A related idea is to modify an initial open-loop trajectory in some purposeful manner in order to improve some performance criteria, based on multiple executions of the trajectory. This general idea is called iterative learning of control (ILC). Abu-Dakka et al. (\cite{Abu-Dakka2012Peg-In-HolePrimitives}) proposed a method for refining PiH insertions in order to minimize contact forces, thus allowing faster executions. Their main goal was also to demonstrate generalization over varying positions of the hole, although they made the major assumption that even the open-loop control trajectory was able to insert the peg, and what remained to be improved was only the magnitude of the contact forces and from there, the speed of insertion. However, as mentioned above, our experience with position estimates obtained from standard industrial machine vision cameras has shown that the associated large errors in position estimation (around 2mm) do not allow successful completion of the trajectory generated by the DMP, even when executed by a compliant controller. Accordingly, this failure makes it impossible to apply ILC methods to improve the controller by minimizing contact forces.  

Another method for modifying the parameters of the DMP directly is to use an RL algorithm that uses trial and error to improve the control policy represented by the DMP. Pastor et al. (\cite{Pastor2009LearningDemonstration}) applied the PI2 RL algorithm to optimize control policies for playing pool and flipping a box using chopsticks. As usual for RL-based methods, both tasks used very highly specialized and task-specific cost functions that were likely the result of extensive experimentation. Furthermore, although the latter task (box flipping) did use force input from pressure sensors mounted on the fingers of the gripper, it is not an assembly task per se, and it is not clear how this general approach can be used for assembly tasks involving contact between multiple parts. Kalakrishnan et al. (\cite{Kalakrishnan2011LearningManipulation}) explored a similar application of the PI2 algorithm to modify DMPs, for manipulation tasks that required force control policies, such as opening a door and grasping a pen. However, again, these tasks needed highly engineered cost functions, and were not assembly tasks.    


